Misalignment vs Topology in Axion-Like Models

Cosmological axions, an important dark matter candidate, are generated when a scalar field with a spontaneously broken O(2) invariance develops an explicitly O(2)-breaking tilt cosmologically, leading to coherent production of long-wavelength modes which could be dark matter. It appears that the production efficiency of this mechanism is low, despite possible production from topological structures. To understand this better, we examine production in O(N) generalizations. In particular we highlight the importance of how fast the explicit O(N)-breaking potential turns on.

==> Ancillary/Code/3Code/pcg-cpp-master/sample/Makefile <==
# 
# PCG Random Number Generation for C++.
# 
# Copyright 2014-2017 Melissa O'Neill <oneill@pcg-random.org>,
#                     and the PCG Project contributors.
#
# SPDX-License-Identifier: (Apache-2.0 OR MIT)
#
# Licensed under the Apache License, Version 2.0 (provided in
# LICENSE-APACHE.txt and at http://www.apache.org/licenses/LICENSE-2.0)
# or under the MIT license (provided in LICENSE-MIT.txt and at
# http://opensource.org/licenses/MIT), at your option. This file may not
# be copied, modified, or distributed except according to those terms.
#
# Distributed on an "AS IS" BASIS, WITHOUT WARRANTY OF ANY KIND, either
# express or implied.  See your chosen license for details.
#
# For additional information about the PCG random number generation scheme,
# visit http://www.pcg-random.org/.
#

TARGETS           = pcg-demo codebook cppref-sample make-partytrick
BINARYOUT_TARGETS = spew use-partytrick

CPPFLAGS += -I../include 
CXXFLAGS += -std=c++11 -O2
CC       = $(CXX)       # Cheat so that linking uses the C++ compiler

all: $(TARGETS)

posix-binaryoutput: spew use-partytrick

clean:
	rm -f *.o $(TARGETS) $(BINARYOUT_TARGETS)

codebook.o: codebook.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
cppref-sample.o: cppref-sample.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
make-partytrick.o: make-partytrick.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
pcg-demo.o: pcg-demo.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
spew.o: spew.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
use-partytrick.o: use-partytrick.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp


==> Ancillary/Code/3Code/pcg-cpp-master/test-high/Makefile <==
# 
# PCG Random Number Generation for C++.
# 
# Copyright 2014-2017 Melissa O'Neill <oneill@pcg-random.org>,
#                     and the PCG Project contributors.
#
# SPDX-License-Identifier: (Apache-2.0 OR MIT)
#
# Licensed under the Apache License, Version 2.0 (provided in
# LICENSE-APACHE.txt and at http://www.apache.org/licenses/LICENSE-2.0)
# or under the MIT license (provided in LICENSE-MIT.txt and at
# http://opensource.org/licenses/MIT), at your option. This file may not
# be copied, modified, or distributed except according to those terms.
#
# Distributed on an "AS IS" BASIS, WITHOUT WARRANTY OF ANY KIND, either
# express or implied.  See your chosen license for details.
#
# For additional information about the PCG random number generation scheme,
# visit http://www.pcg-random.org/.
#

TARGETS           = \
    check-pcg8_once_insecure check-pcg8_oneseq_once_insecure               \
    check-pcg16_once_insecure check-pcg16_oneseq_once_insecure check-pcg32 \
    check-pcg32_c1024 check-pcg32_c1024_fast check-pcg32_c64               \
    check-pcg32_c64_fast check-pcg32_c64_oneseq check-pcg32_fast           \
    check-pcg32_k1024 check-pcg32_k1024_fast check-pcg32_k16384            \
    check-pcg32_k16384_fast check-pcg32_k2 check-pcg32_k2_fast             \
    check-pcg32_k64 check-pcg32_k64_fast check-pcg32_k64_oneseq            \
    check-pcg32_once_insecure check-pcg32_oneseq                           \
    check-pcg32_oneseq_once_insecure check-pcg32_unique check-pcg64        \
    check-pcg64_c1024 check-pcg64_c1024_fast check-pcg64_c32               \
    check-pcg64_c32_fast check-pcg64_c32_oneseq check-pcg64_fast           \
    check-pcg64_k1024 check-pcg64_k1024_fast check-pcg64_k32               \
    check-pcg64_k32_fast check-pcg64_k32_oneseq check-pcg64_once_insecure  \
    check-pcg64_oneseq check-pcg64_oneseq_once_insecure check-pcg64_unique \
    check-pcg128_once_insecure check-pcg128_oneseq_once_insecure

# special flags for some compilers
CPPFLAGS_clang++ += \
	-Weverything \
	-Wno-unknown-warning-option \
	-Wno-c++98-compat \
	-Wno-c++98-compat-pedantic \
	-Wno-date-time \
	-Wno-undef \
	-Wno-header-hygiene \
	-Wno-unused-macros

CPPFLAGS += -I../include -Wall -Wextra $(CPPFLAGS_$(CXX))
CXXFLAGS += -std=c++11
CC       = $(CXX)       # Cheat so that linking uses the C++ compiler

all: $(TARGETS)

test: $(TARGETS)
	sh run-tests.sh

clean:
	rm -f *.o $(TARGETS)
	rm -rf actual

pcg-test-noadvance.o: pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
pcg-test.o: pcg-test.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg8_once_insecure.o: check-pcg8_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg8_oneseq_once_insecure.o: check-pcg8_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg16_once_insecure.o: check-pcg16_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg16_oneseq_once_insecure.o: check-pcg16_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32.o: check-pcg32.cpp pcg-test.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg32_c1024.o: check-pcg32_c1024.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_c1024_fast.o: check-pcg32_c1024_fast.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg32_c64.o: check-pcg32_c64.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_c64_fast.o: check-pcg32_c64_fast.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_c64_oneseq.o: check-pcg32_c64_oneseq.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg32_fast.o: check-pcg32_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k1024.o: check-pcg32_k1024.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k1024_fast.o: check-pcg32_k1024_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k16384.o: check-pcg32_k16384.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k16384_fast.o: check-pcg32_k16384_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k2.o: check-pcg32_k2.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k2_fast.o: check-pcg32_k2_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k64.o: check-pcg32_k64.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k64_fast.o: check-pcg32_k64_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k64_oneseq.o: check-pcg32_k64_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_once_insecure.o: check-pcg32_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_oneseq.o: check-pcg32_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_oneseq_once_insecure.o: check-pcg32_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_unique.o: check-pcg32_unique.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64.o: check-pcg64.cpp pcg-test.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg64_c1024.o: check-pcg64_c1024.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_c1024_fast.o: check-pcg64_c1024_fast.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg64_c32.o: check-pcg64_c32.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_c32_fast.o: check-pcg64_c32_fast.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_c32_oneseq.o: check-pcg64_c32_oneseq.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg64_fast.o: check-pcg64_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k1024.o: check-pcg64_k1024.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k1024_fast.o: check-pcg64_k1024_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k32.o: check-pcg64_k32.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k32_fast.o: check-pcg64_k32_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k32_oneseq.o: check-pcg64_k32_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_once_insecure.o: check-pcg64_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_oneseq.o: check-pcg64_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_oneseq_once_insecure.o: check-pcg64_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_unique.o: check-pcg64_unique.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg128_once_insecure.o: check-pcg128_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg128_oneseq_once_insecure.o: \
  check-pcg128_oneseq_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp


==> Ancillary/Code/4Code/pcg-cpp-master/sample/Makefile <==
# 
# PCG Random Number Generation for C++.
# 
# Copyright 2014-2017 Melissa O'Neill <oneill@pcg-random.org>,
#                     and the PCG Project contributors.
#
# SPDX-License-Identifier: (Apache-2.0 OR MIT)
#
# Licensed under the Apache License, Version 2.0 (provided in
# LICENSE-APACHE.txt and at http://www.apache.org/licenses/LICENSE-2.0)
# or under the MIT license (provided in LICENSE-MIT.txt and at
# http://opensource.org/licenses/MIT), at your option. This file may not
# be copied, modified, or distributed except according to those terms.
#
# Distributed on an "AS IS" BASIS, WITHOUT WARRANTY OF ANY KIND, either
# express or implied.  See your chosen license for details.
#
# For additional information about the PCG random number generation scheme,
# visit http://www.pcg-random.org/.
#

TARGETS           = pcg-demo codebook cppref-sample make-partytrick
BINARYOUT_TARGETS = spew use-partytrick

CPPFLAGS += -I../include 
CXXFLAGS += -std=c++11 -O2
CC       = $(CXX)       # Cheat so that linking uses the C++ compiler

all: $(TARGETS)

posix-binaryoutput: spew use-partytrick

clean:
	rm -f *.o $(TARGETS) $(BINARYOUT_TARGETS)

codebook.o: codebook.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
cppref-sample.o: cppref-sample.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
make-partytrick.o: make-partytrick.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
pcg-demo.o: pcg-demo.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
spew.o: spew.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
use-partytrick.o: use-partytrick.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp


==> Ancillary/Code/4Code/pcg-cpp-master/test-high/Makefile <==
# 
# PCG Random Number Generation for C++.
# 
# Copyright 2014-2017 Melissa O'Neill <oneill@pcg-random.org>,
#                     and the PCG Project contributors.
#
# SPDX-License-Identifier: (Apache-2.0 OR MIT)
#
# Licensed under the Apache License, Version 2.0 (provided in
# LICENSE-APACHE.txt and at http://www.apache.org/licenses/LICENSE-2.0)
# or under the MIT license (provided in LICENSE-MIT.txt and at
# http://opensource.org/licenses/MIT), at your option. This file may not
# be copied, modified, or distributed except according to those terms.
#
# Distributed on an "AS IS" BASIS, WITHOUT WARRANTY OF ANY KIND, either
# express or implied.  See your chosen license for details.
#
# For additional information about the PCG random number generation scheme,
# visit http://www.pcg-random.org/.
#

TARGETS           = \
    check-pcg8_once_insecure check-pcg8_oneseq_once_insecure               \
    check-pcg16_once_insecure check-pcg16_oneseq_once_insecure check-pcg32 \
    check-pcg32_c1024 check-pcg32_c1024_fast check-pcg32_c64               \
    check-pcg32_c64_fast check-pcg32_c64_oneseq check-pcg32_fast           \
    check-pcg32_k1024 check-pcg32_k1024_fast check-pcg32_k16384            \
    check-pcg32_k16384_fast check-pcg32_k2 check-pcg32_k2_fast             \
    check-pcg32_k64 check-pcg32_k64_fast check-pcg32_k64_oneseq            \
    check-pcg32_once_insecure check-pcg32_oneseq                           \
    check-pcg32_oneseq_once_insecure check-pcg32_unique check-pcg64        \
    check-pcg64_c1024 check-pcg64_c1024_fast check-pcg64_c32               \
    check-pcg64_c32_fast check-pcg64_c32_oneseq check-pcg64_fast           \
    check-pcg64_k1024 check-pcg64_k1024_fast check-pcg64_k32               \
    check-pcg64_k32_fast check-pcg64_k32_oneseq check-pcg64_once_insecure  \
    check-pcg64_oneseq check-pcg64_oneseq_once_insecure check-pcg64_unique \
    check-pcg128_once_insecure check-pcg128_oneseq_once_insecure

# special flags for some compilers
CPPFLAGS_clang++ += \
	-Weverything \
	-Wno-unknown-warning-option \
	-Wno-c++98-compat \
	-Wno-c++98-compat-pedantic \
	-Wno-date-time \
	-Wno-undef \
	-Wno-header-hygiene \
	-Wno-unused-macros

CPPFLAGS += -I../include -Wall -Wextra $(CPPFLAGS_$(CXX))
CXXFLAGS += -std=c++11
CC       = $(CXX)       # Cheat so that linking uses the C++ compiler

all: $(TARGETS)

test: $(TARGETS)
	sh run-tests.sh

clean:
	rm -f *.o $(TARGETS)
	rm -rf actual

pcg-test-noadvance.o: pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
pcg-test.o: pcg-test.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg8_once_insecure.o: check-pcg8_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg8_oneseq_once_insecure.o: check-pcg8_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg16_once_insecure.o: check-pcg16_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg16_oneseq_once_insecure.o: check-pcg16_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32.o: check-pcg32.cpp pcg-test.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg32_c1024.o: check-pcg32_c1024.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_c1024_fast.o: check-pcg32_c1024_fast.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg32_c64.o: check-pcg32_c64.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_c64_fast.o: check-pcg32_c64_fast.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_c64_oneseq.o: check-pcg32_c64_oneseq.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg32_fast.o: check-pcg32_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k1024.o: check-pcg32_k1024.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k1024_fast.o: check-pcg32_k1024_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k16384.o: check-pcg32_k16384.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k16384_fast.o: check-pcg32_k16384_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k2.o: check-pcg32_k2.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k2_fast.o: check-pcg32_k2_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k64.o: check-pcg32_k64.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k64_fast.o: check-pcg32_k64_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k64_oneseq.o: check-pcg32_k64_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_once_insecure.o: check-pcg32_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_oneseq.o: check-pcg32_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_oneseq_once_insecure.o: check-pcg32_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_unique.o: check-pcg32_unique.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64.o: check-pcg64.cpp pcg-test.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg64_c1024.o: check-pcg64_c1024.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_c1024_fast.o: check-pcg64_c1024_fast.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg64_c32.o: check-pcg64_c32.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_c32_fast.o: check-pcg64_c32_fast.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_c32_oneseq.o: check-pcg64_c32_oneseq.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg64_fast.o: check-pcg64_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k1024.o: check-pcg64_k1024.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k1024_fast.o: check-pcg64_k1024_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k32.o: check-pcg64_k32.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k32_fast.o: check-pcg64_k32_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k32_oneseq.o: check-pcg64_k32_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_once_insecure.o: check-pcg64_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_oneseq.o: check-pcg64_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_oneseq_once_insecure.o: check-pcg64_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_unique.o: check-pcg64_unique.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg128_once_insecure.o: check-pcg128_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg128_oneseq_once_insecure.o: \
  check-pcg128_oneseq_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp


==> Ancillary/Code/5Code/5Code/pcg-cpp-master/sample/Makefile <==
# 
# PCG Random Number Generation for C++.
# 
# Copyright 2014-2017 Melissa O'Neill <oneill@pcg-random.org>,
#                     and the PCG Project contributors.
#
# SPDX-License-Identifier: (Apache-2.0 OR MIT)
#
# Licensed under the Apache License, Version 2.0 (provided in
# LICENSE-APACHE.txt and at http://www.apache.org/licenses/LICENSE-2.0)
# or under the MIT license (provided in LICENSE-MIT.txt and at
# http://opensource.org/licenses/MIT), at your option. This file may not
# be copied, modified, or distributed except according to those terms.
#
# Distributed on an "AS IS" BASIS, WITHOUT WARRANTY OF ANY KIND, either
# express or implied.  See your chosen license for details.
#
# For additional information about the PCG random number generation scheme,
# visit http://www.pcg-random.org/.
#

TARGETS           = pcg-demo codebook cppref-sample make-partytrick
BINARYOUT_TARGETS = spew use-partytrick

CPPFLAGS += -I../include 
CXXFLAGS += -std=c++11 -O2
CC       = $(CXX)       # Cheat so that linking uses the C++ compiler

all: $(TARGETS)

posix-binaryoutput: spew use-partytrick

clean:
	rm -f *.o $(TARGETS) $(BINARYOUT_TARGETS)

codebook.o: codebook.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
cppref-sample.o: cppref-sample.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
make-partytrick.o: make-partytrick.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
pcg-demo.o: pcg-demo.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
spew.o: spew.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
use-partytrick.o: use-partytrick.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp


==> Ancillary/Code/5Code/5Code/pcg-cpp-master/test-high/Makefile <==
# 
# PCG Random Number Generation for C++.
# 
# Copyright 2014-2017 Melissa O'Neill <oneill@pcg-random.org>,
#                     and the PCG Project contributors.
#
# SPDX-License-Identifier: (Apache-2.0 OR MIT)
#
# Licensed under the Apache License, Version 2.0 (provided in
# LICENSE-APACHE.txt and at http://www.apache.org/licenses/LICENSE-2.0)
# or under the MIT license (provided in LICENSE-MIT.txt and at
# http://opensource.org/licenses/MIT), at your option. This file may not
# be copied, modified, or distributed except according to those terms.
#
# Distributed on an "AS IS" BASIS, WITHOUT WARRANTY OF ANY KIND, either
# express or implied.  See your chosen license for details.
#
# For additional information about the PCG random number generation scheme,
# visit http://www.pcg-random.org/.
#

TARGETS           = \
    check-pcg8_once_insecure check-pcg8_oneseq_once_insecure               \
    check-pcg16_once_insecure check-pcg16_oneseq_once_insecure check-pcg32 \
    check-pcg32_c1024 check-pcg32_c1024_fast check-pcg32_c64               \
    check-pcg32_c64_fast check-pcg32_c64_oneseq check-pcg32_fast           \
    check-pcg32_k1024 check-pcg32_k1024_fast check-pcg32_k16384            \
    check-pcg32_k16384_fast check-pcg32_k2 check-pcg32_k2_fast             \
    check-pcg32_k64 check-pcg32_k64_fast check-pcg32_k64_oneseq            \
    check-pcg32_once_insecure check-pcg32_oneseq                           \
    check-pcg32_oneseq_once_insecure check-pcg32_unique check-pcg64        \
    check-pcg64_c1024 check-pcg64_c1024_fast check-pcg64_c32               \
    check-pcg64_c32_fast check-pcg64_c32_oneseq check-pcg64_fast           \
    check-pcg64_k1024 check-pcg64_k1024_fast check-pcg64_k32               \
    check-pcg64_k32_fast check-pcg64_k32_oneseq check-pcg64_once_insecure  \
    check-pcg64_oneseq check-pcg64_oneseq_once_insecure check-pcg64_unique \
    check-pcg128_once_insecure check-pcg128_oneseq_once_insecure

# special flags for some compilers
CPPFLAGS_clang++ += \
	-Weverything \
	-Wno-unknown-warning-option \
	-Wno-c++98-compat \
	-Wno-c++98-compat-pedantic \
	-Wno-date-time \
	-Wno-undef \
	-Wno-header-hygiene \
	-Wno-unused-macros

CPPFLAGS += -I../include -Wall -Wextra $(CPPFLAGS_$(CXX))
CXXFLAGS += -std=c++11
CC       = $(CXX)       # Cheat so that linking uses the C++ compiler

all: $(TARGETS)

test: $(TARGETS)
	sh run-tests.sh

clean:
	rm -f *.o $(TARGETS)
	rm -rf actual

pcg-test-noadvance.o: pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
pcg-test.o: pcg-test.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg8_once_insecure.o: check-pcg8_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg8_oneseq_once_insecure.o: check-pcg8_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg16_once_insecure.o: check-pcg16_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg16_oneseq_once_insecure.o: check-pcg16_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32.o: check-pcg32.cpp pcg-test.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg32_c1024.o: check-pcg32_c1024.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_c1024_fast.o: check-pcg32_c1024_fast.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg32_c64.o: check-pcg32_c64.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_c64_fast.o: check-pcg32_c64_fast.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_c64_oneseq.o: check-pcg32_c64_oneseq.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg32_fast.o: check-pcg32_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k1024.o: check-pcg32_k1024.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k1024_fast.o: check-pcg32_k1024_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k16384.o: check-pcg32_k16384.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k16384_fast.o: check-pcg32_k16384_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k2.o: check-pcg32_k2.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k2_fast.o: check-pcg32_k2_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k64.o: check-pcg32_k64.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k64_fast.o: check-pcg32_k64_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_k64_oneseq.o: check-pcg32_k64_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_once_insecure.o: check-pcg32_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_oneseq.o: check-pcg32_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_oneseq_once_insecure.o: check-pcg32_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg32_unique.o: check-pcg32_unique.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64.o: check-pcg64.cpp pcg-test.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg64_c1024.o: check-pcg64_c1024.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_c1024_fast.o: check-pcg64_c1024_fast.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg64_c32.o: check-pcg64_c32.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_c32_fast.o: check-pcg64_c32_fast.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_c32_oneseq.o: check-pcg64_c32_oneseq.cpp \
  pcg-test-noadvance.cpp ../include/pcg_random.hpp \
  ../include/pcg_extras.hpp ../include/pcg_uint128.hpp
check-pcg64_fast.o: check-pcg64_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k1024.o: check-pcg64_k1024.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k1024_fast.o: check-pcg64_k1024_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k32.o: check-pcg64_k32.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k32_fast.o: check-pcg64_k32_fast.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_k32_oneseq.o: check-pcg64_k32_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_once_insecure.o: check-pcg64_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_oneseq.o: check-pcg64_oneseq.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_oneseq_once_insecure.o: check-pcg64_oneseq_once_insecure.cpp \
  pcg-test.cpp ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg64_unique.o: check-pcg64_unique.cpp pcg-test-noadvance.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg128_once_insecure.o: check-pcg128_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp
check-pcg128_oneseq_once_insecure.o: \
  check-pcg128_oneseq_once_insecure.cpp pcg-test.cpp \
  ../include/pcg_random.hpp ../include/pcg_extras.hpp \
  ../include/pcg_uint128.hpp

